Don't Blame the Model, Verify the Data: An Evaluation of SMT-based Dataset Verification (Extended Version)

The EU AI Act mandates that datasets for high-risk machine learning (ML) systems meet strict quality criteria such as soundness and bias mitigation. While Satisfiability Modulo Theory (SMT) solving offers a formal approach to verifying these properties, its scalability in realistic ML settings remains unexplored. To bridge this gap, this work presents the first large-scale empirical study of SMT-based dataset verification on two real-world ML datasets. We systematically evaluate how solver performance is shaped by three key dimensions: the type of data-quality property, the specification style, and the dataset encoding strategy. Our findings demonstrate that SMT-based verification is feasible for practical scenarios, but each dimension shapes it: the property type sets the tractability limit, the specification style drives scalability (exceeding $2{,}000{\times}$ for aggregate properties), and the encoding strategy has a systematic effect, with extracted feature columns performing best.

==> sections/02_Background.tex <==
\textbf{Preliminaries.}
SMT solving extends propositional satisfiability through theories such as linear integer arithmetic or arrays.
Given  a set of assertions, an SMT solver returns 
\texttt{sat} if a satisfying assignment exists, \texttt{unsat} if it does not, and \texttt{unknown} if it cannot determine the result within its resource limits.
In~\cite{dsverification}, a tabular dataset is encoded as an array $D[i][j]$, where $i$ indicates a record and $j$ a feature, 
together with a separate array for labels, and a property is expressed as a formula over these arrays. 
Verification reduces to checking whether the conjunction of the dataset encoding and the property formula is satisfiable. 
%The approach was reproducibly evaluated on a synthetic dataset of ten records with
%four properties and for the property well-distributedness, 
%the solver consistently returned \texttt{unknown}.
